On Mixing Eventual and Strong Consistency: Acute Cloud Types

In this article we study the properties of distributed systems that mix eventual and strong consistency. We formalize such systems through acute cloud types (ACTs), abstractions similar to conflict-free replicated data types (CRDTs), which by default work in a highly available, eventually consistent fashion, but which also feature strongly consistent operations for tasks which require global agreement. Unlike other mixed-consistency solutions, ACTs can rely on efficient quorum-based protocols, such as Paxos. Hence, ACTs gracefully tolerate machine and network failures also for the strongly consistent operations. We formally study ACTs and demonstrate phenomena which are neither present in purely eventually consistent nor strongly consistent systems. In particular, we identify temporary operation reordering, which implies interim disagreement between replicas on the relative order in which the client requests were executed. When not handled carefully, this phenomenon may lead to undesired anomalies, including circular causality. We prove an impossibility result which states that temporary operation reordering is unavoidable in mixed-consistency systems with sufficiently complex semantics. Our result is startling, because it shows that apparent strengthening of the semantics of a system (by introducing strongly consistent operations to an eventually consistent system) results in the weakening of the guarantees on the eventually consistent operations.

==> a2-bayou_proof.tex <==
%auto-ignore

\subsection{Bayou -- proofs of correctness} \label{sec:proofs:bayou}

\endinput
In this section we 
% formally 
analyze the correctness properties that the 
(modified) Bayou and similar protocols guarantee. We outline the %a detailed 
system model necessary to conduct the formal proofs. Then we study 
the correctness of Bayou.

\begin{comment}
Since, as we have already shown, the basic Bayou protocol exhibits circular 
causality, it does not satisfy neither $\BEC$ nor $\FEC$. Thus, we shift our 
attention to the modified protocol. Although it does not suffer from circular 
causality, it still features temporary operation reordering, what makes it not 
$\BEC$-compliant. However, below we show that it does satisfy $\FEC$. We also 
show that, in case of strong operations, it guarantees sequential consistency 
($\SC(\strong, \FF)$).
\end{comment}

\begin{comment}
\subsection{Box properties} \label{sec:analysis:box}

Before we analyze the Bayou protocol, let us begin with the formal description 
of the semantics of the Box as an isolated element. As it was stated earlier 
the Box encapsulates the state of a system after locally executing a sequence 
of operations. Below we provide a succint formal framework to reason about the 
responses obtained from the Box.

\noindent \textbf{Traces and call-patterns.}
Let \emph{trace} be a sequence of operations invoked on the Box of the 
following form: $\langle o_1, o_2, ... \rangle$, where each $o_i$ is either a 
request execution with a return value $e(r_x) \rightarrow v$, or a request 
rollback $r(r_x)$, where $r_x$ is the request. Let \emph{call-pattern} be a 
similar sequence, just without the return values of request execution calls.
We say that a trace $\alpha$ and a call-pattern $\beta$ correspond to each 
other, if $\beta$ can be obtained from $\alpha$ simply be removing return 
values. A call-pattern is exec-only if it does not contain any rollback 
operations. For an exec-only call-pattern we can replace $e(r_x)$ with $r_x$, 
and treat the call-pattern simply as a sequence of requests.

A call-pattern $\alpha$ is \emph{reducible} to a call-pattern $\beta$, if and 
only if:
\begin{itemize}
\item $\alpha = \pre \cdot \langle e(r_x), r(r_y) \rangle \cdot \suf$, where 
$r_x = r_y$, and $\beta = \pre \cdot \suf$, or
\item $\alpha$ is reducible to $\alpha'$ which is reducible to $\beta$.
\end{itemize}

If a call-pattern $\alpha$ is reducible to an exec-only call-pattern $\beta$, 
then we say that $\beta$ is a \emph{normalization} of $\alpha$. Note that there 
may exist only a single normalization of any call-pattern.

A call-pattern $\alpha$ is \emph{valid} if it is exec-only, or it has a 
normalization.

We can see that all call-patterns of the Box in Bayou are valid, and that the 
list $\executed \cdot \reverse(\toBeRolledBack)$ at any given time identifies, 
either the current call-pattern, or its normalization. To understand why, 
consider the following facts:
\begin{itemize}
\item requests are executed only if $\toBeRolledBack = \epsilon$ (an empty 
sequence),
\item whenever a request is executed it is added to the $\executed$ list, 
\item in the $\adjustExecution$ function, some requests may be moved from the 
$\executed$ list to the end of the $\toBeRolledBack$ list, thus not changing 
their position in the combined list $\executed \cdot \reverse(\toBeRolledBack)$,
\item whenever a request is rolled back, it is taken from the head of the 
$\toBeRolledBack$ list and removed from it; thus the request is removed from 
the end of the combined list, which is equivalent to adding a rollback 
operation and reducing the call-pattern to a normalization.
\end{itemize}

Now let us define one more time reducibility, but this time for traces. A trace 
$\alpha$ is reducible to a trace $\beta$, if and only if:
\begin{itemize}
\item $\alpha = \pre \cdot \langle e(r_x) \rightarrow v, r(r_y) \rangle \cdot 
\suf$, where $r_x = r_y$, and $\beta = \pre \cdot \suf$, or
\item $\alpha$ is reducible to $\alpha'$ which is reducible to $\beta$.
\end{itemize}
Note that this definition is more demanding than in case of call-patterns, 
because return values of execute operations in $\pre$ and $\suf$ have to be 
retained. It means that not only the reduced execute and rollback operations 
have to match, but also that removing them does not influence return values of 
subsequent operations.

\noindent \textbf{Consistency.}
Let $\EE$ be the set of all traces produced by the Box.
We say that the Box is \emph{consistent}, if and only if:
\begin{itemize}
\item for each valid call-pattern, there exists a single corresponding trace in 
$\EE$, and
\item for each trace $\alpha \in \EE$ and every trace $\beta$ to which 
$\alpha$ is reducible, $\beta \in \EE$.
\end{itemize}
The first point guarantees that the responses of the Box are deterministic 
(e.g. if $\langle e(r_1) \RA v_1, e(r_2) \RA v_2 \rangle \in \EE$, then 
$\langle e(r_1) \RA v_1, e(r_2) \RA v_3 \rangle \not\in \EE$, where $v_2 \neq 
v_3$). The second point ensures that the Box, upon rolling a request back,
returns to the state on which the request was executed. To understand why, 
consider the following example: assume that $\alpha = \langle e(r_1) \RA v_1, 
e(r_2) \RA v_2 \rangle \in \EE$ and $\alpha' = \langle e(r_1) \RA v_1, e(r_x) 
\RA v_x, r(r_x), e(r_2) \RA v_y \rangle \in \EE$. Because of the second point, 
the normalization of $\alpha'$, $\beta = \langle e(r_1) \RA v_1, e(r_2) \RA v_y 
\rangle \in \EE$. But then, because both $\alpha$ and $\beta$ correspond to the 
same call-pattern, and because of the first point, $v_y = v_2$. Thus, whenever 
a rollback happens we can treat the original trace and its normalization, as 
equal in terms of the Box' responses to subsequent operations, just as if the 
rolled back request was never executed.

\noindent \textbf{Return value semantics.}
The above definition enforces quite useful semantics of the Box, yet a 
consistent Box may still return nonsensical values from the execute operation 
(e.g. a Box that returns $\bot$ for any request execution is trivially 
consistent). We have to put additional requirements on the return values so 
that they are consistent with the implemented type $\FF$.

For any trace $\alpha$, let $\beta$ be the normalization of the corresponding 
call-pattern, $E_\alpha$ be the set of requests in $\beta$, $\eo_\alpha 
\subseteq E_\alpha \times E_\alpha$ be the order in which requests are 
enumerated in $\beta$, and $\op : \Request \longrightarrow \ops(\FF)$ be 
a function that for any request $r = (\timestamp, \dot, \strongOp, \opn)$ 
returns the invoked operation $r.\opn$. We say that the Box implements a type 
$\FF$, if and only if, for any trace $\alpha \in \EE$, and any execute 
operation $e(r) \rightarrow v$ in $\alpha$, $v = \FF(\op(r), (E_\gamma, 
\eo_\gamma, \eo_\gamma, \op))$, where $\gamma$ is the prefix of $\alpha$ up to 
(but excluding) the operation $e(r) \rightarrow v$.
Example: $\alpha = \langle e(r_1) \RA v_1, e(r_2) \RA v_2, r(r_2), e(r_3) \RA 
v_3, r(r_3), e(r_4) \RA v_4, e(r_5) \RA v_5 \rangle$; to compute $v_3$ we use 
$E_\gamma = \{ r_1 \}$ and $\eo_\gamma = \langle r_1 \rangle$; to compute $v_5$ 
we use $E_\gamma = \{ r_1, r_4 \}$ and $\eo_\gamma = \langle r_1, r_4 \rangle$. 

Note that $\eo_\gamma$ is the order of requests in the normalization of the 
call-pattern corresponding with $\gamma$, thus in Bayou it is equivalent to the 
list $\executed \cdot \reverse(\toBeRolledBack)$ at the time of the operation 
$e(r) \rightarrow v$.

\noindent \textbf{Implementation.}
The Box in Figure~\ref{alg:box} is both consistent and implements the type 
$\FF$ (given that the code for $r.\opn$ is deterministic and correct according 
to the type $\FF$). It assumes that each operation can be specified as a 
composition of read and write operations on registers together with some local 
computation. The assumption is sensible, as the operations are executed 
locally, in a sequential manner, and thus no stronger primitives than registers 
are necessary. The Box keeps an undo log which allows it to revoke the effects 
of any request executed so far. The provided Box implementation is only 
illustratory, a specialized implementation can be proposed for a specific type 
$\FF$.

{\renewcommand\small{\scriptsize}%        
    \input{algorithms/box_alg.tex}
}

We assume that the Box used in the Bayou protocol is always consistent and 
implements the type $\FF$.
\end{comment}

\subsubsection{The $\boxx$ properties} \label{sec:analysis:box}

% {\renewcommand\small{\scriptsize}%        
%     \input{algorithms/box_alg.tex}
% }

% The $\boxx$ encapsulates the state of a system after locally executing a 
% sequence of operations. 
Take the list of requests that were executed on the $\boxx$, and remove the 
requests which were rolled back; we call the resulting sequence $\alpha$ the 
current trace of the $\boxx$. Since the $\boxx$ encapsulates the state of the 
system after locally executing and revoking requests, we require that the 
$\boxx$'s responses are consistent with a deterministic serial execution of 
$\alpha$ as specified by the type specification $\FF$. In Bayou, $\alpha = 
\executed \cdot \reverse(\toBeRolledBack)$, because:
% To understand why, consider the following facts:
\begin{itemize}
\item requests are executed only if $\toBeRolledBack$ is empty,
% $= \epsilon$ (an empty sequence),
\item whenever a request is executed it is added to the $\executed$ list,
thus it is appended to the end of $\alpha$,
\item in the $\adjustExecution$ function, some requests 
% may be 
move from the 
$\executed$ list to the end of the $\toBeRolledBack$ list, thus not changing 
their position in $\alpha$,
\item whenever a request is rolled back, it is removed from the head of the 
$\toBeRolledBack$ list, and thus removed from the end of $\alpha$, consistently 
with the definition of a trace.
\end{itemize}

% Below we provide a succint formal framework to reason 
% about the responses obtained from the $\boxx$.
% We require the $\boxx$ is \emph{consistent} and implements the type $\FF$. 
% Informally, it means that its responses are deterministic, a rollback of some 
% request $r$ revokes the $\boxx$ to the state as if 
% $r$ was never executed and $\boxx$'s responses are coherent with $\FF$.

\begin{comment}

Algorithm~\ref{alg:box} shows a pseudocode of \StateObject, a referential 
implementation of $\boxx$ for arbitrary $\FF$ (a specialized one can be 
used for a specific $\FF$). We assume that each operation can be specified as a 
composition of read and write operations on registers together with some local 
computation. The assumption is sensible, as the operations are executed 
locally, in a sequential manner, and thus no stronger primitives than registers 
(such as CAS, fetch-and-add, etc.) are necessary. The \StateObject keeps an 
undo log which allows it to revoke the effects of any request executed so far. 
% Intuitively, given that the code for $r.\opn$ 
% is deterministic and correct according to $\FF$, the algorithm satisfies our 
% requirements.
% is both consistent and implements $\FF$. 
% We skip the formal proof of the correctness due to space contstraints.


\end{comment}






\begin{comment}
\subsection{The $\boxx$ properties} \label{sec:analysis:box}

Before we analyze the Bayou protocol, let us begin with the formal description 
of the semantics of the $\boxx$ as an isolated element. As it was stated 
earlier the $\boxx$ encapsulates the state of a system after locally executing 
a sequence of operations. 
% Below we provide a succint formal framework to reason 
% about the responses obtained from the $\boxx$.
We require the $\boxx$ to be \emph{consistent} and to implement type $\FF$. 
Informally, consistency means, that the $\boxx$' responses are deterministic, 
and that rollback of some request $r$ returns the $\boxx$ to the state as if 
$r$ was never executed. The $\boxx$ implements type $\FF$ if its responses are 
coherent with $\FF$. 
% Below we explain both terms in more detail.
% Below we succintly describe what we mean by it.

\noindent \textbf{Implementation.}
In Figure~\ref{alg:box} we present a referential implementation of the $\boxx$.
It is both consistent and implements the type $\FF$ (given that the code for 
$r.\opn$ is deterministic and correct according to the type $\FF$). It assumes 
that each operation can be specified as a composition of read and write 
operations on registers together with some local computation. The assumption is 
sensible, as the operations are executed locally, in a sequential manner, and 
thus no stronger primitives than registers are necessary. The $\boxx$ keeps an 
undo log which allows it to revoke the effects of any request executed so far. 
The provided $\boxx$ implementation is only illustratory, a specialized 
implementation can be proposed for a specific type $\FF$.

{\renewcommand\small{\scriptsize}%        
    \input{algorithms/box_alg.tex}
}

\noindent \textbf{Traces and normalizations.}
Let us now provide a succint formal framework to reason about the responses 
obtained from the $\boxx$. Let \emph{trace} be a sequence of operations invoked 
on the $\boxx$ of the following form: $\langle o_1, o_2, ... \rangle$, where 
each $o_i$ is either a request execution with a return value $e(r_x) 
\rightarrow v$, or a request rollback $r(r_x)$, where $r_x$ is the request. 

We reduce traces, by removing neighboring execute and rollback elements in a 
recursive manner. If a trace $\alpha$ can be reduced so that it does not 
contain any rollback operations, then we say it is \emph{valid}, and we obtain 
its \emph{normalization} $n(\alpha)$, by replacing each $e(r_x) \rightarrow v$ 
in the reduced $\alpha$ with $r_x$.

We can see that all traces of the $\boxx$ in Bayou are valid, and that the list 
$\executed \cdot \reverse(\toBeRolledBack)$ at any given time identifies the 
normalization of the current trace. To understand why, consider the following 
facts:
\begin{itemize}
\item requests are executed only if $\toBeRolledBack = \epsilon$ (an empty 
sequence),
\item whenever a request is executed it is added to the $\executed$ list, 
\item in the $\adjustExecution$ function, some requests may be moved from the 
$\executed$ list to the end of the $\toBeRolledBack$ list, thus not changing 
their position in the combined list $\executed \cdot \reverse(\toBeRolledBack)$,
\item whenever a request is rolled back, it is taken from the head of the 
$\toBeRolledBack$ list and removed from it; thus the request is removed from 
the end of the combined list, which is equivalent to adding a rollback 
operation and reducing the trace.
\end{itemize}

\noindent \textbf{Consistency.}
Let $\EE$ be the set of all valid traces produced by the $\boxx$. We say that 
the $\boxx$ is \emph{consistent}, if and only if, for any $\alpha, \beta \in 
\EE$: $n(\alpha) = n(\beta)$ implies that, either $\alpha$ can be reduced to 
$\beta$, or vice versa. Thus, no two traces can exist in $\EE$ with the same 
normalization, but different return values. Example: $\bullet$~if $\langle 
e(r_1) \RA 5, e(r_2) \RA 6 \rangle \in \EE$, then $\langle e(r_1) \RA 5, e(r_2) 
\RA 7 \rangle \not\in \EE$; $\bullet$~if $\langle e(r_1) \RA 5, r(r_1), e(r_2) 
\RA 1 \rangle \in \EE$, then $\langle e(r_2) \RA 2 \rangle \not\in \EE$; 
$\bullet$~however, if $\langle e(r_1) \RA 5, r(r_1), e(r_2) \RA 1 \rangle \in 
\EE$, then $\langle e(r_2) \RA 1 \rangle \in \EE$.

\noindent \textbf{Return value semantics.}
The above definition enforces quite useful semantics of the $\boxx$, yet a 
consistent $\boxx$ may still return nonsensical values from the execute 
operation (e.g. a $\boxx$ that returns $\bot$ for any request execution is 
trivially consistent). We have to put additional requirements on the return 
values so that they are coherent with the type $\FF$.

Let $E(\alpha)$ be the set of requests in $n(\alpha)$, and $\op : \Request 
\longrightarrow \ops(\FF)$ be a function that for any request $r = (\timestamp, 
\dot, \strongOp, \opn)$ returns the invoked operation $r.\opn$. We say that the 
$\boxx$ implements a type $\FF$, if and only if, for any trace $\alpha \in 
\EE$, and any execute operation $e(r) \rightarrow v$ in $\alpha$, we take 
$\gamma$ to be the prefix of $\alpha$ up to (but excluding) the operation $e(r) 
\rightarrow v$, and $v = \FF(\op(r), (E(\gamma), n(\gamma), n(\gamma), 
\op))$.\footnote{Notice that we use here a normalization $n(\gamma)$, which is 
a sequence of requests, as a total order relation over requests and substitute 
it for $\vis$ and $\ar$ in the context.} 
Note that $n(\gamma)$ is the normalization of the current trace at the time of 
the operation $e(r) \rightarrow v$. Thus in Bayou it is equivalent to the list 
$\executed \cdot \reverse(\toBeRolledBack)$.
Example: $\alpha = \langle e(r_1) \RA v_1, e(r_2) \RA v_2, r(r_2), e(r_3) \RA 
v_3, r(r_3), e(r_4) \RA v_4, e(r_5) \RA v_5 \rangle$; $\bullet$~to compute 
$v_3$ we use $E(\gamma) = \{ r_1 \}$ and $n(\gamma) = \langle r_1 \rangle$; 
$\bullet$~to compute $v_5$ we use $E(\gamma) = \{ r_1, r_4 \}$ and $n(\gamma) = 
\langle r_1, r_4 \rangle$. 
\end{comment}









\subsubsection{Bayou in stable runs} \label{sec:analysis:stable}

Now we 
% SHORT
% proceed to 
formally characterize the modified Bayou's behaviour in 
stable runs. 

% \begin{theorem}
% Bayou satisfies $\FEC(\weak, \FF) \wedge \SC(\strong, \FF)$ in stable runs for 
% arbitrary $\FF$.
% \end{theorem}

\bayoustable*

\begin{proof}
\todo{Update with linearizability.}
For an arbitrary fair execution $G$, we obtain its history $H = 
(E, \op, \rval, \rb, \sss, \lvl)$. We construct the relations $\vis$, $\ar$, and 
$\perc(e)$ for each $e \in E$, which we then use together with $H$ to form an 
abstract execution $A$. We need to show that $A \models \FEC(\weak, \FF) \wedge 
\SC(\strong, \FF)$. However, for $\FEC$ we show a stronger result, $A 
\models \FEC(\weak, \FF) \wedge \FEC(\strong, \FF)$, to help us with a 
later proof.

% SHORT
% Let us introduce some notation, 
We define the following functions over $E$:
\begin{itemize}
\item $\req(e)$ -- the request issued in the event $e$, 
\item $\tob(e)$ -- whether $\req(e)$ was $\tobcast$ ($\tob(e) = \true \iff 
(\tobcast\ \req(e)) \in \sent(e)$),
\item $\tobdel(e)$ -- whether $\req(e)$ was $\tobdeliver$ed by any replica 
($\tobdel(e) = \true \iff \tobNo(\req(e)) \neq \bot$).
\end{itemize}
Note that $\tob(e) = \true$ only for updating events ($\op(e) \not\in 
\readonlyops(\FF)$) and strong \RO ones ($\op(e) \in \readonlyops(\FF) 
\wedge \lvl(e) = \strong$). Also notice that in stable runs the following 
holds: $\tob(e) \iff \tobdel(e)$.

First, note that we can compare lexicographically requests generated (and thus 
also messages exchanged) in Bayou -- a request is a tuple of values. The first 
element of the tuple is the timestamp, while the second one is a dot, which 
itself is a pair. Dots, uniquely identify requests, as the 
$\currentEventNumber$ grows strictly monotonically on each replica with each 
$\invoke$ event, and the replica number $i$ is unique for any replica. Thus, 
each request is unique (the function $\req$ is a bijection), and all requests 
induce a total order over $E$.

For an event $e \in E$, such that $\rval(e) \neq \nabla$, let $\ret(e)$ denote 
the event $r \in G$, in which the response $\rval(e)$ was computed. We can 
define $r$ formally as follows:
\begin{itemize}
\item $r = e$, if $\lvl(e) = \weak$, or
\item $r$ is an $\execute$ event, such that $\rep(r) = \rep(e)$ and $\req(e)$ 
is the head of $\pre(r).\toBeExecuted$.
\end{itemize}
The second point unambiguously identifies a single event. This is 
because strong operations in the modified protocol are disseminated only using 
TOB. When a strong request is $\tobdeliver$ed, it is added to the $\committed$ 
list, and thus 
% SHORT
% Once a request is added to the $\committed$ list, 
it cannot be rolled 
back.
% SHORT
% and thus 
Hence, a request that is only $\tobcast$ will be executed exactly once 
by each replica.

\noindent \textbf{Arbitration.}
The final arbitration order for $\tobcast$ events (updating or strong 
\RO) in Bayou is determined by the order imposed by TOB. Although 
\RO operations, by definition, do not influence the return values of any 
other operation, for completeness, the weak \RO events also have to be 
included in $\ar$. We establish the total order of all operations by mixing the 
TOB order for events which were $\tobcast$, and the inherent order induced by 
the requests themselves: $e \raar e' \iff$
\begin{itemize}
\item $\tobNo(\req(e)) < \tobNo(\req(e'))$, or
\item $\tobdel(e) \wedge \tob(e') \wedge \neg \tobdel(e')$, or
\item $\tob(e) \wedge \neg \tobdel(e) \wedge \tob(e') \wedge \neg \tobdel(e') 
\wedge \req(e) < \req(e')$, or
\item $(\neg \tob(e) \vee \neg \tob(e')) \wedge \req(e) < \req(e')$.
\end{itemize}
(The first point applies only if $\tobdel(e) \wedge \tobdel(e')$.)

% (obviously, by the properties of TOB, $\ar$ is a total order).

However, when operations are executed and replicas compute the responses which 
are returned to the clients, the \emph{perceived arbitration order} $\perc(e)$ 
is used instead of $\ar$.

Now we define the total order $\perc(e)$: $\bullet$~we take the current trace 
of the $\boxx$ which was used when computing $\rval(e)$ as the base; 
$\bullet$~we put all the $\tobcast$ events, which are not in the trace, 
after $e$ (relatively in the $\ar$ order); $\bullet$~we insert some weak 
\RO requests before $e$ (if they precede $e$ in $\ar$); $\bullet$~and we 
insert some weak \RO requests after $e$ (if they are preceded by $e$ in 
$\ar$). This way $e$ is preceded in $\perc(e)$ only by events which were 
actually used to compute the return value $\rval(e)$, and some weak \RO 
events, which precede $e$ in $\ar$, because e.g. they have a lower timestamp.

Let $\exec(e) = \alpha$, where $\alpha$ is the current trace of the $\boxx$ 
in event $\ret(e)$. Thus, $\alpha = \pre(\ret(e)).\executed \cdot 
\reverse(\pre(\ret(e)).\toBeRolledBack)$. Note that $\exec(e)$ contains only 
requests which were $\tobcast$.

\newcommand{\poshe}{\pos_{\hat{e}}}

Let $\exec'(e) = \exec(e) \cdot \req(e)$. Note that $\exec'(e)$ may contain a 
weak \RO request, only if $e$ is one itself. Let $\poshe(e')$ be the 
position of request $r = \req(e')$ in the list $\exec'(\hat{e})$, or $\bot$ if 
$r$ is not on the list. 

The definition of $\perc(\hat{e})$ is as follows:
$e \rapar{\hat{e}} e' \iff$
\begin{itemize}
\item $\poshe(e) < \poshe(e')$, or
\item $\poshe(e) \neq \bot \wedge \poshe(e') = \bot \wedge 
\tob(e')$, or
\item $\poshe(e') = \bot \wedge \neg \tob(e') \wedge e \raar 
e'$, or
\item $\poshe(e) = \bot \wedge \neg \tob(e) \wedge e \raar e'$, or
\item $\poshe(e) = \bot \wedge \poshe(e') = \bot \wedge e 
\raar e'$.
\end{itemize}
In the above definition two events are ordered in the $\perc(\hat{e})$ 
according to their position on $\exec'(\hat{e})$ list, if they both exist on 
the list. All the events that are not on the list, but could have been, because 
they were $\tobcast$, are ordered after all the events that are on the list. 
All the weak \RO events (which are not present in the list, and not 
$\tobcast$), are ordered relatively to the events on the list according to 
$\ar$. Similarly, any two events which are both not on the list (irregardless 
whether they were $\tobcast$), are ordered according to $\ar$. Clearly, 
$\perc(\hat{e})$ is a total order over $E$.

It is also easy to see that $\perc(\hat{e})$, with each subsequent event 
$\hat{e}$, converges to $\ar$. This is caused by the fact that each message 
$\tobdeliver$ed puts some request $r$ in the $\committed$ list, and for any 
two events $e,e'$, such that $\req(e), \req(e') \in \pre(\hat{e}).\committed$, 
$e \rapar{\hat{e}} e' \iff e \raar e'$ (the $\committed$ list which is a prefix 
of $\exec'(\hat{e})$ is ordered by $\tobNo$, similarly to $\ar$). Moreover, for 
any two events $e,e'$, such that $\neg \tob(e) \vee \neg \tob(e')$, $e 
\rapar{\hat{e}} e' \iff e \raar e'$ (weak \RO events are, by definition, 
ordered in $\perc(\hat{e})$ relatively to other events based on $\ar$). Hence, 
whether an event $e$ was $\tobcast$, or not, eventually (for infinitely many 
events $\hat{e}$) for any $e' \in E$, $e \rapar{\hat{e}} e' \iff e \raar e'$, 
and $e' \rapar{\hat{e}} e \iff e' \raar e$. 
% in $\perc(\hat{e})$ it will be ordered at the exactly same position as 
% according to $\ar$, 
Thus, $A \models \CPERC(\weak) \wedge \CPERC(\strong)$.

\noindent \textbf{Visibility.}
We define the visibility relation through the perceived arbitration order. 
% SHORT
% Simply, 
An event $e$ is visible to some other event $e'$ if it is perceived by 
$e'$ to happen before it: $e \ravis e' \iff e \rapar{e'} e'$. Note that, $e 
\ravis e'$, if and only if, $\req(e) \in \exec(e')$, or $\req(e) \not\in 
\exec(e') \wedge \req(e) < \req(e')$. 
$A \models \EV$, because for every event $e$, eventually $e 
\rapar{\hat{e}} e'$ (as shown above), thus $e \rapar{e'} e'$, thus $e 
\ravis e'$.
% \begin{comment}
% % SHORT
% % Clearly, 
% Eventual visibility is satisfied 
% ($A \models \EV$), because each request
% % SHORT
% % which is 
% $\tobcast$ by some replica, 
% eventually gets $\tobdeliver$ed by all replicas. Then, it becomes part of the 
% $\pre(\hat{e}).\committed$ list for each subsequent event $\hat{e}$. On the 
% other hand, an event which is not $\tobcast$, will have a lower timestamp 
% than every other request from some point on, and thus is also ordered before 
% the other requests in $\perc(\hat{e})$ and visible to them.
% \end{comment}

% Clearly, eventual visibility is satisfied 
% ($A \models \EV$), because each request which is $\tobdeliver$ed by some 
% replica, eventually gets $\tobdeliver$ed by all replicas. Then, it becomes 
% part 
% of the $\pre(\hat{e}).\committed$ list for each subsequent event $\hat{e}$. 
% On 
% the other hand, an event which is never $\tobdeliver$ed, will have a lower 
% timestamp than every other request from some point on, and thus also ordered 
% before the other requests in $\perc(\hat{e})$ and visible to them.

It was shown in Section~\ref{sec:bayou_modified} that the modified protocol 
does not suffer from the circular causality anomaly, which means that the 
relation $\hb$ must be acyclic, and thus $A \models \NCC$.

\noindent \textbf{Return values.}
To prove that $A \models \FEC(\weak, \FF) \wedge \FEC(\strong, \FF)$ it remains 
to show that $A \models \FRVAL(\weak, \FF) \wedge \FRVAL(\strong, \FF)$, i.e. 
that for any $e \in E$, $\rval(e) = \FF(\op(e), c)$, where $c = \fcontext(A, e) 
= (V, \vis, \perc(e), \op)$ and $V = \vis^{-1}(e)$. Let $c' = (V', \vis, 
\perc(e), \op)$ be a context obtained from $c$ be removing all events $e'$ from 
$V$, such that $\op(e') \in \readonlyops(\FF) \wedge \lvl(e) = \weak$. By the 
definition of a \RO operation $\FF(\op(e), c) = \FF(\op(e), c')$. Notice, 
that $e' \in V' \iff \req(e') \in \exec(e)$. It is easy to see now that $c'$ is 
isomorphic with $c'' = (V'', \exec(e), \exec(e), \op')$, where $V'' = \{ r | 
\req^{-1}(r) \in V' \}$ and $\op'(r) = r.\opn$, for any request $r$. Thus, 
$\FF(\op(e), c') = \FF(\op(e), c'')$. Since we know that the $\boxx$'s 
responses are consistent with $\FF$,
% consistent and implements type $\FF$, 
and that $\exec(e)$ is the current trace of the $\boxx$ when $\rval(e)$ is 
computed, $\rval(e) = \FF(\op(e), c'') = \FF(\op(e), c)$.

\noindent \textbf{Strong operations.}
For strong operations we have to additionally prove that $A \models 
\SO(\strong) \wedge \SA(\strong) \wedge \RVAL(\strong, \FF)$. Let us begin with 
$\SO(\strong)$. Let $e$ be some event such that $\lvl(e) = \strong$. Since 
$\tobdel(e)$, $\rval(e) \neq \nabla$ ($e$ is not pending). We have to 
show that for any event $e'$, $e' \ravis e \iff e' \raar e$. Obviously, 
$\exec(e) = \pre(\ret(e)).\committed$. For any event $e'$ which was $\tobcast$, 
$e' \in \exec(e) \iff \tobNo(e') < \tobNo(e) \iff e' \raar e$. Thus, $e' 
\rapar{e} e \iff e' \raar e$. For any event $e'$ which was not $\tobcast$, by 
definition, $e' \rapar{e} e \iff e' \raar e$. Therefore, $e' \ravis e \iff e' 
\raar e$. Also, notice that $\perc(e) = \ar$.

Let us consider $\SA(\strong)$. Let $e$ be some event such that $\lvl(e) = 
\strong$. It is easy to see, that for any event $e'$, such that $e' \raso e$, 
if $e'$ was $\tobcast$, then $\tobNo(e') < \tobNo(e)$ (by the FIFO 
requirement), on the other hand, if $e'$ was not $\tobcast$ then, $\req(e') < 
\req(e)$. Thus $e' \raar e$. %, and $e' \ravis e$.

$\RVAL(\strong, \FF)$ is automatically satisfied, because $\FRVAL(\strong, 
\FF)$ is satisfied and for each event $e$ such that $\lvl(e) = \strong$, 
$\perc(e) = \ar$.
Thus, Bayou satisfies $\FEC(\weak, \FF) \wedge \SC(\strong, \FF)$ in stable 
runs. \qedsymbol
\end{proof}

\subsubsection{Bayou in asynchronous runs} \label{sec:analysis:async}

% \begin{theorem}
% Bayou satisfies $\FEC(\weak, \FF)$ but does not satisfy $\FEC(\weak, \FF) 
% \wedge \SC(\strong, \FF)$ in asynchronous runs for arbitrary $\FF$.
% \end{theorem}

\bayouasynchronous*

\begin{proof}
\todo{Update with linearizability.}
In the stable runs, the following holds: $\tob(e) \iff \tobdel(e)$. However, in 
asynchronous runs this is no longer true. Some $\tobcast$ events might get 
$\tobdeliver$ed, while others not.

The definitions of $\vis$, $\ar$, $\perc$ are the same as in stable runs: 
they do not require assuming that $\tob(e) \iff \tobdel(e)$.
% Moreover, some of the predicates are satisfied, by the same reasoning as in 
% the previous subsection. We may only need to look closer at $\CPERC(\weak) 
% \wedge \CPERC(\strong)$, $\EV$ and $\RVAL(\weak, \FF)$.

To prove that $A \models \CPERC(\weak) \wedge \CPERC(\strong)$, we can use the 
same reasoning as we did in stable runs, but we have to take into account that 
some $\tobcast$ events might not get $\tobdeliver$ed, thus their requests will 
not end up in the $\committed$ list. For each such event $e$ ($\tob(e) \wedge 
\neg \tobdel(e)$), there are two possibilities: either $e$ is a weak updating 
event, and thus $\req(e)$ will be eventually $\rbdeliver$ed by all replicas, 
and ended up in the $\tentative$ list, thus becoming part of the 
$\exec(\hat{e})$ for each subsequent event $\hat{e}$, or it is a strong 
operation which is pending. In the former case, both in $\ar$, and in 
$\perc(\hat{e})$, $e$ will be ordered after any $\tobdeliver$ed event, and will 
be ordered relatively to all other events by the request order. In the latter 
case, the same applies. Thus eventually, for any $e' \in E$, $e \rapar{\hat{e}} 
e' \iff e \raar e'$, and $e' \rapar{\hat{e}} e \iff e' \raar e$.

% To prove that $A \models \EV$, notice that for every event $e$, such that 
% $\tob(e) \wedge \neg \tobdel(e)$, eventually $e \rapar{\hat{e}} e'$ (as shown 
% above), thus $e \rapar{\hat{e}} \hat{e}$, thus $e \ravis \hat{e}$.

$\EV$, $\NCC$ and $\FRVAL(\weak, \FF)$ are satisfied by the same reasoning as 
in case 
of stable runs. Thus
% SHORT
% , we have shown that 
$A \models \FEC(\weak, \FF)$.

Now let us consider $\FRVAL(\strong, \FF)$. Unfortunately, some strong events 
may be pending, so $\rval(e) = \nabla$, and thus $\rval(e) \neq 
\FF(\op(r), \fcontext(A, e))$.\footnote{However, if $\rval(e) \neq \nabla$, 
then $\rval(e) = \FF(\op(r), \fcontext(A, e))$.} This 
means, that neither $\FEC(\strong, \FF)$, nor $\SC(\strong, \FF)$ can be 
satisfied. Thus, Bayou satisfies only $\FEC(\weak, \FF)$ in asynchronous 
runs. \qedsymbol
\end{proof}










==> a3-actnnc_proof.tex <==
\subsection{\ACTnnc\ -- proofs of correctness} \label{sec:proofs:annc}

\actnncstable*

\begin{proof}
\end{proof}

\actnncasynchronous*

\begin{proof}
\end{proof}

Before we dive into details let us make one observation. In \ACTnnc clients do 
not explicitely maintain separate sessions. However we know that each replica 
executes all operations sequentially and thus we can define the replica order 
relation, which must be respected by $\rb \cap \sss$. Formally, replica order 
($\ro$) is a union of total orders on each replica such that for any two events 
$e, e'$ executed on replica $R_i$ if $e$ was executed before $e'$, $e \raro e'$. 
Hence, in the proof we will rely on $\ro$ rather than to $\rb \cap \sss$.

\begin{lemma}
\ACTnnc satisfies $\BEC(\FFnnc, \weak)$ in both stable and asynchronous runs.
\end{lemma}

\begin{proof}
In order to prove the lemma, we need to assume some history $H = (E, \op, \rval, 
\rb, \sss, \lvl)$ and show that we can construct an abstract execution 
$A = (H, \vis, \ar, \perc)$, such that $A \models \EV(\weak) \wedge \NCC(\weak) 
\wedge \RVAL(\weak, \FFnnc)$.

Let us first define two auxilary relations. The first one is the \emph{message 
delivery} relation $\del$: $\forall e,e' \in E$, $e \radel e'$ if and only if 
the replica that executed $\op(e')$ delivered all messages sent in $\op(e)$.
Obviously in case of \ACTnnc $\op(e)$ could be only $\add$ or $\subtract$.

% The second relation is the \emph{knowledge dominance} relation $\kd$: 
% $\forall e,e' \in E, e \rakd e' \iff \del^{-1}(e) \subseteq \del^{-1}(e') 
% \wedge e \ro e'$. If $e \rakd e'$, it means that the replica that executed 
% $\op(e')$, prior the execution of $\op(e')$ delivered all messages that were 
% delivered by the replica that executed $\op(e)$ prior to execution of 
% $\op(e)$.
%  
% ($e'$ already delivered all messaged delivered 



We can now start with constuction of the visibility relation ($\vis$):
\begin{myeq}
\forall e,e' \in E : \Big(e \radel e' &\\
  \vee (lvl(e) = lvl(e') = weak \wedge e \raso e') &\\
  \vee del^{-1}(e) \subset del^{-1}(e')\Big) &\\
  & \Rightarrow e \ravis e'
\end{myeq}

Intuitively, $\vis$ is a union of the $\del$ relation, the $\ro$ relation for 
weak operations and one more relation that 


\end{proof}
\endinput






Claim: ANNC satisfies EV(weak)

we need to show that for each event e in E there exist an infinite number of
weak events e' such that e \ravis e'. We need to consider three cases:
- if op(e) = add, e rbcasts some message and in a fair execution these messages
  will be eventually rbdelivered by all processes; hence from some point on
  on every replica, every weak operation will observe e; since we consider
  a fair execution, each replica will perform an infinite number of operations
- if op(e) = subtract then we have two cases to consider
  * TOB terminates and at least one (correct) replica tobdeliveres messages
    sent in e; then by our assumptions of fair executions, all replicas
    eventually tobdeliver messages sent in e, which leads to a similar argument
    as above
  * TOB cannot terminate (e.g., in an unstable run) and then e is pending;
    hence there is no e'' such that e \rarb e'' and e' needs not to observe e
- if op(e) = get, let S = del^{-1}(e) (S includes rbcast as well as tobcast
  messages); as we argued above, all these messages will eventually reach
  each replica and each replica executes and infinite number of events []  

Claim: ANNC satisfies NNC(weak)

NNC(weak) = acyclic(hb \cap (L x L)) 
= acyclic((\so \cup \vis)^+ \cap (L x L))
= acyclic(((\rb \cap \sss) \cup \vis)^+ \cap (L x L))

where L = ...

Since we consider the \ro relation, we will show by a contradiction that 
acyclic(\ro \cup \vis)^+ \cap (L x L)).

Assume otherwise: there exists a set $W = \{ e_1, e_2, ..., e_n \}$ of events 
in which weak operations were invoked, such that $e_1 \rarel e_2 \rarel ... 
\rarel e_n \rarel e_1$, where $\rarel$ is either $\ro$ or $\vis$. Let $W$ be a 
minimal set of this kind. If $W$ contains only events, such that for each two 
$e,e' \in W$, either $e \raro e'$ or $e' \raro e$, then there is no cycle $\hb 
\cap (L \times L)$ because $\ro$ is a total order and thus is obviousy acyclic. 
Hence, there must be $e, e' \in W$, such that $e \ravis e'$ and $e \not\raso 
e'$ and $e' \not\raso e$. Then either:
- e \radel e': since there is a cycle in (\ro \cup \vis)^+ \cap (L x L) then 
either:
  * e' \radel e
  * del^{-1}(e') \subset del^{-1}(e)
- del^{-1}(e) \subset del^{-1}(e')
  * 
By our construction of \vis, each pair e_i \rarel e_j is such that e_j 
is aware of at least the same set of 
  
  
======================
  
it is clear that by incorporating first two requirements, we ensure that
an updating operation executing on some replica recognizes all updating
operations that the replica knows about (received appropriate messages)

the last requirement is necessary to ensure eventual visibility of 
read-only evens

hb = (so u vis)+  // cap L x L
  
- will subtract be able to observe earlier adds and subtracts? yes
- will get be able to observe earlier adds and subtracts? yes
- read-only operations
  
we start with constructing \vis

general idea - key elements:
- subtracts observe only earlier subtracts
- adds observe all updating ops 
  * executed earlier on the same replica
  * whose messages reached the replica before executing the add
- gets observe all updating ops 
  * whose messages reached the replica before executing the add

- we need to ensure also eventual visibility of events
-> kazda operacja obserwuje te ready, ktore obserwowaly co najmniej taki stan?
-> del_msg : E -> 2^E - a function that for each event e returns a set of 
  updating events e', such that message issued by e' has been delivered 
  by the replica executing e, before it executed e

  
substract operation:
- execution of \op(e) results in issuing a tob message m
- if at least one replica tobdelivers such m, then the order of m relative 
  to all other tobdelivered messages is set. Hence, we define tobno(e)
  equal to the total number of all tobdelivered messages that were tobdelivered
  by the replica that first tobdelivered m (if some other replica also 
  tobdelivers m, the numbers will be equal by the properties of TOB).
- otherwise tobno(e) = \bot, is undefined
- \forall e,e' \in E : op(e) = op(e') = subtract \wedge tobno(e) \neq \bot 
  \wedge tobno(e') \neq \bot : e \ravis_sub e' \iff tobno(e) < tobno(e')
  
add operation:
- we define the visibility of add operations in two steps
- add operation e observes all weak adds on the same replica
- formally let sadd be a relation on U x U, where U = { e | e \in E : 
  opn(e) = add }, such that 
  \forall e,e' in E : e saad e' \iff e \so \e' \cap (U x U)
- e observes all updating operations whose messages have been delivered
  (either by RB or TOB) to replica on which e is executed prior to e's
  execution; 
- formally let msg be a relation on V x E, where V = { e | e \in E : opn(e) 
  \not\in \readonlyops(FFnnc) }, such that e \ramsg e' iff the replica that 
  executed e' delivered (through RB or TOB) any message broacast in e
- forall e \in E, e' in U : e \ravis_add e' \iff (e \saad e') \cup (e \msg e')

get operations:
- we reuse the msg relation
- 


vis = vis_sub \cup vis_add \cup vis_get


we start with constructing \ar

first for updating ops e \not\in \readonlyops(\FFnnc)
- we start building ar by having all e with tobno(e) defined arranged 
  according to tobno, in the ascending order
  \forall e,e' in E : \tobno(e) \neq \bot \wedge \tobno(e') \neq bot 
  e \raar e' \iff tobno(e) < tobno(e')
# no gaps in tob (by properties of tob)
- in a stable run we're done with the updating ops, because for every 
  updating op a message is tobcast, and by the definiton of stable runs,
  each such m is everntually delivered by every (correct) process
- in an asynchronous run we've got an infinite number of updating ops e
  for which tobno(e) is undefined; we append them to our sequence
  according to their ids (but they should be (currentEventNo, i)), sorted
  lexographically 
- no we need to add the get operations
- let e be any get operation and e' be an updating op such that 
- let e \in \readonlyops(FFnnc); if \exists e', e'' \in E : 
  tobno(e') \neq \bot \wedge tobno(e'') \neq \bot, e' \raar e \raar e'';
  'in between' such e', e'' we arrange all such e according to replica id
  and program order within that replica id
- otherwise, we append after the last e'' such that tobno(e'') \neq \bot


























==> a4-redblue.tex <==
\subsection{Guarantees of ACTs vs RedBlue consistency} \label{sec:redblue}

Let us now discuss in more detail RedBlue consistency \cite{LPC+12} and 
highlight the differences between this approach and ours. We do so by showing 
an example of a system that satisfies RedBlue consistency but provides
weaker guarantees than some ACTs that implement the same operations.

Recall the $\FFseq$ replicated data type which exported two operations: 
$\app(s)$, which appends string $s$ to an ever-growing sequence of characters, 
and $\rd()$, which allows us to output the current value of the sequence. 
Let the $\app()$ operation appear in two variants: the strongly consistent 
\emph{red} variant (the $\redapp()$ operation) and the eventually consistent 
\emph{blue} variant (the $\blueapp()$ operation). Let $\rd()$ appear only 
in the blue variant (the $\bluerd()$ operation). In 
Algorithm~\ref{alg:seq_redblue} we provide a pseudocode of a system 
implementing these operations and which works in the RedBlue consistency model.

RedBlue consistency requires that all blue operations commute with all other 
operations, i.e., the state of the replica does not depend on the order in 
which the operations are applied locally. Obviously, in a straightforward 
implementation, in which each replica stores a local copy of a ever-growing 
string, a $\blueapp()$ operation does not commute with any other operation (it 
commutes only with the $\bluerd()$ operation, and not with the other 
$\blueapp()$ operations nor the $\redapp()$ operations). Hence, we follow the 
\emph{generator-shadow operations} scheme introduced in \cite{LPC+12} and split 
$\blueapp()$ into a side-effect free generator operation and a globally 
commutative shadow operation (we treat the $\redapp()$ operation in a similar 
fashion). The generator prepares a $\Request$ structure that includes the 
string $s$ to be appended to the end of the sequence and the current timestamp. 
The structure defines a newly issued shadow operation, which is either red 
or blue, to match the colour of the generator operation. During the execution 
of the shadow operation, in the $\mathit{appendShadow}(\Request: r)$ function, 
the executing replica increases its local logical clock $\lc$, to ensure that 
the subsequently issued $\blueapp()$ or $\redapp()$ operations will be 
serialized after the operation described by $r$. Then, the replica adds $r$ to 
the $\delReqs$ set. Each time the $\bluerd()$ operation is invoked, the 
$\delReqs$ set is analyzed to construct the current value of the sequence. The 
strings received in the $\Request$ structures are arbitrated firstly using the 
$\lc$ field and then using the $s$ field (lexicographically). Due to the nature 
of RedBlue consistency, the generated $\Request$ structures are distributed 
among replicas in a way that respects the causal ordering guarantees among blue 
operations as well as ensures the total order of delivery of all red operations 
across all replicas (it can be accomplished, e.g., using the Gemini scheme 
described in the same paper as RedBlue consistency). Note that the provided 
generator and shadow operations are \emph{correct} as defined in \cite{LPC+12}, 
i.e., the generator operation is side-effect free, and the shadow operation 
produces the same effect as the original $\app$ operation would have, when 
executed on the same state on which the generator was executed.

{\renewcommand\small{\footnotesize}%        
    \input{algorithms/seq_redblue.tex}
}

\begin{figure*}[t]
\center
% \begin{multicols*}{2}
% \begin{column}{0.3\textwidth}
% \end{column}
% \begin{column}{0.7\textwidth}
% \columnbreak
\begin{tabular}{p{5in}}
{\input{histories/redblue.tex}}\\
\end{tabular}
% \end{column}
% \end{multicols*}
\caption{A execution demonstrating the lack of operation stabilization even for 
red operations in a system that satisfies RedBlue consistency. The system 
implements $\FFseq$ and supports both strongly consistent red operations 
($\redapp()$) and causally consistent blue operations ($\blueapp()$, 
$\bluerd()$). The implementation of all the operations is given in 
Algorithm~\ref{alg:seq_redblue}.}
\label{fig:redblue}
\end{figure*}

It is easy to see that a system constructed in such a way satisfies all the 
requirements of the RedBlue model, which we informally outline below:
\begin{itemize}
\item all operations are non-blocking,
% \item all generator operations are side-effect free,
\item all operations which perform changes to the replica commute with each 
other,
\item as replicas execute operations, replicas' states converge to the the same 
state,
\item causal relationships between operations are respected, and
\item all replicas share a common order of all red shadow operations.
\end{itemize}
However, despite all the guarantees provided by RedBlue consistency, and 
the necessity of solving distributed consensus to ensure the total order of all 
red (shadow) operations across replicas, the counter-intuitive execution 
depicted in Figure~\ref{fig:redblue} is possible:
\begin{itemize}
\item $R_1$ executes $\blueapp(a)$ operation, while $R_2$ executes $\redapp(b)$,
\item $R_2$ subsequently executes $\bluerd() \rightarrow b$,
% since in the RedBlue model causal dependencies between operations are always 
% respected, $\bluerd()$ can return $b$ only if $\blueapp(a)$ was not visible 
% to $\redapp(b)$,
\item because in the RedBlue model causal dependencies between operations are 
always respected, and $\blueapp(a)$ operation was not visible to the $\bluerd() 
\rightarrow b$ operation, it could neither have been visible to the strongly 
consistent $\redapp(b)$ operation, 
\item one could assume that $b$ has to be the first element of the end sequence,
\item however, the end sequence is $ab$, because $\blueapp(a)$ has been issued 
with a lower $\lc$ than $\redapp(b)$.
\end{itemize}
Now imagine an implementation of the same operations, but based on, e.g., 
Bayou. In order to ensure the strongly consistent semantics of the $\redapp()$ 
operation, a replica would not admit a new operation until the invoked 
$\redapp()$ is stabilized. When a \emph{strong} operation $\opn$ (here, 
$\redapp()$) is executed, the set of operations that precede $\opn$ cannot 
change. Thus, subsequently issued operations observe a stable prefix of the 
sequence which includes the effects of the $\redapp()$ operation. On the other 
hand, the RedBlue model does not guarantee stabilization of red operations: the 
order of red operations relative to blue operations is always subject to 
change, i.e., arbitrarily many blue operations may later appear to have been 
executed prior to the red operation.

The example shows that in the RedBlue model, unlike in ACTs, solving 
distributed consensus does not translate into having \emph{fully-fledged} 
strongly consistent semantics of the red operations. The consequences of such 
behaviour are not apparent when we use the formalism of the RedBlue model, 
which abstracts away from the return values of operations and focuses solely on 
replica states. In this sense, our framework allows one to conduct more 
in-depth analysis.




\endinput


==> algorithms/act_counter.tex <==
\begin{algorithm}[t] 
\caption{Acute non-negative counter (\ACTnnc) for replica $R_i$}
\label{alg:actnnc}  
% \algsetup{linenosize=\tiny}
  \footnotesize
% \vspace{-0.15cm}
% \begin{multicols*}{2}
\begin{algorithmic}[1]
% \State{\Struct $\Message$($\type$ : ${\{}$ ADD, SUBTRACT ${\}}$, $\value$ : int)}
\State{\Struct $\Request$($\type$ : ${\{}$ADD, SUBTRACT${\}}$, $\val$ : int, \par
         \hskip 3.2em $\idd$ : pair$\langle$int, int$\rangle$)}
\State{\Var $\wi$, $\si$, $\sd$, $\currentEventNumber$ : int} \label{alg:actpc:vars}
\State{\Var $\requestsAwaitingResponse$ : set$\langle$pair$\langle$int, int$\rangle\rangle$}
\Procedure{$\add$}{$\val$ : int} \LineComment{weak operation} \label{alg:actpc:add}
    \State{$\currentEventNumber = \currentEventNumber + 1$}
    \State{$\wi = \wi + \val$}
    \State{$r = \Request($ADD, $\val, (i, \currentEventNumber))$}
    \State{$\rbcast(r)$} \label{alg:actpc:addrb}
    \State{$\tobcast(r)$} \label{alg:actpc:addtob}
%     \State{\Return $\ok$}
\EndProcedure
\Function{$\subtract$}{$\val$ : int} \LineComment{strong operation} \label{alg:actpc:subtract}
    \State{$\currentEventNumber = \currentEventNumber + 1$}
%     \State{\Var $\idd = (i, \currentEventNumber)$}
    \State{$r = \Request($SUBTRACT, $\val, (i, \currentEventNumber))$}
    \State{$\tobcast(r)$}
    \State{$\requestsAwaitingResponse = \requestsAwaitingResponse \cup \{ \idd \}$}
\EndFunction
\Upon{$\rbdeliver$}{$r$ : $\Request($ADD, $\val, \idd)$} 
    \If{$r.\dot.\mathit{first} = i$}\LineComment{$r$ issued locally}
        \State{\Return}
    \EndIf
    \State{$\wi = \wi + \val$}
\EndUpon
\Upon{$\tobdeliver$}{$r$ : $\Request($ADD, $\val, \idd)$} 
    \State{$\si = \si + \val$}
\EndUpon
\Upon{$\tobdeliver$}{$r$ : $\Request($SUBTRACT, $\val, \idd)$} 
    \State{\Var $\res = \si \geq \sd + \val$} \label{alg:actpc:subcalcstart}
    \If{$\res$}
        \State{$\sd = \sd + \val$} \label{alg:actpc:subcalcend}
    \EndIf
    \If{$\idd \in \requestsAwaitingResponse$}
        \State{$\requestsAwaitingResponse = \requestsAwaitingResponse \setminus \{ \idd \}$}
        \State{return $\res$ to client} 
    \EndIf
\EndUpon
\Function{$\get$()}{} \LineComment{read-only, weak operation} \label{alg:actpc:get}
    \State{\Return $\maxx(\wi, \si) - \sd$} \label{alg:actpc:getc}
\EndFunction
\end{algorithmic}
\end{algorithm}

\endinput



\Function{$\rollback$}{$r$ : $\Request$}
    \State{\Var $\undoMap = \undoLog[r]$}
    \For{$(k,v) \in \undoMap$}
        \State{$\db[k] = v$}
        \State{$\undoLog = \undoLog \setminus (r, \undoMap)$}
    \EndFor
\EndFunction
\end{algorithmic}
% \end{multicols*}
% \vspace{-0.4cm}
\end{algorithm}

\endinput




==> algorithms/bayou_alg2.tex <==
% \newcommand{\previous}{\mathsf{previous}}
% \newcommand{\subsequent}{\mathsf{subsequent}}
% 
% \newcommand{\newTentative}{\mathsf{newTentative}}
% \newcommand{\inOrder}{\mathsf{inOrder}}
% \newcommand{\outOfOrder}{\mathsf{outOfOrder}}
% 
% \newcommand{\head}{\mathsf{head}}
% \newcommand{\tail}{\mathsf{tail}}

\begin{algorithm*}%[p] 
\caption{Modification to Bayou protocol that prevents circular causality and improves fault-tolerance}
\label{alg:bayou}  
% \algsetup{linenosize=\tiny}
%   \footnotesize
  \scriptsize
\vspace{-0.15cm}
\begin{multicols*}{2}
\begin{algorithmic}[1]
\State{\Struct $\Request$($\timestamp$ : int, $\dot$ : pair$\langle$int, int$\rangle$, \par
         \hskip 4.7em $\strongOp$ : boolean, $\opn$ : $\ops(\FF)$)}

\Operator{$<$}{$\rr : \Request$, $\rr' : \Request$}
    \State{\Return $(\rr.\timestamp, \rr.\dot) < (\rr'.\timestamp, \rr'.\dot)$}
\EndOperator

\State{\Var $\boxx$ : \StateObject} \label{alg:bayou:box}
\State{\Var $\currentEventNumber$ : int}
\State{\Var $\committed$, $\tentative$ : list$\langle\Request\rangle$}
\State{\Var $\executed$, $\toBeExecuted$, $\toBeRolledBack$ : list$\langle\Request\rangle$}
\State{\Var $\requestsAwaitingResponse$ : map$\langle\Request, \Response\rangle$}
% \State{\Var $\lastResponse$ : $\Response$}

% \Upon{$\invoke$}{$\opn$ : $\ops(\FF)$, $\strongOp$ : boolean} \label{alg:bayou:invoke}
%     \State{$\currentEventNumber = \currentEventNumber + 1$} \label{alg:bayou:currInc}
%     \State{\Var $r = \Request(\currentTime, (i, \currentEventNumber), \strongOp, \opn)$}
%     \State{$\rbcast(\langle\ISSUE, r\rangle)$} \label{alg:bayou:rbcast}
%     \State{$\tobcast(r)$} \label{alg:bayou:tobcast}
%     \State{\Call{$\adjustTentativeOrder$}{$r$}} \label{alg:bayou:adjustTentativeOrder_early}
%     \State{$\requestsAwaitingResponse.\pput(r, \bot)$}
% \EndUpon

\Upon{$\invoke$}{$\opn$ : $\ops(\FF)$, $\strongOp$ : boolean}
    \If{$\neg\strongOp \wedge \opn \in \readonlyops(\FF)$}
        \State{\Var $\response = \boxx.\execute(\opn)$}
        \State{return $\response$ to client}
    \Else
        \State{$\currentEventNumber = \currentEventNumber + 1$}
        \State{\Var $r = \Request(\currentTime, (i, \currentEventNumber), \strongOp, \opn)$}
        \If{$\neg\strongOp$}
    %         \State{\algemph{\Var $\response = \boxx.\execute(r)$}}
            \State{\Var $\response = \boxx.\execute(r)$}
            \State{return $\response$ to client}
%             \If{$\opn \not\in \readonlyops(\FF)$}
            \State{$\boxx.\rollback(r)$}
            \State{$\rbcast(r)$}
            \State{$\tobcast(r)$}
            \State{\Call{$\adjustTentativeOrder$}{$r$}}
%             \EndIf
        \Else
            \State{$\requestsAwaitingResponse.\pput(r, \bot)$}
            \State{$\tobcast(r)$}
        \EndIf
    \EndIf
\EndUpon

\Procedure{$\adjustTentativeOrder$}{$r$ : $\Request$} \label{alg:bayou:adjustTentativeOrder}
    \State{\Var $\previous = [ x | x \in \tentative \wedge x < r ]$}
    \State{\Var $\subsequent = [ x | x \in \tentative \wedge r < x ]$}    
    \State{$\tentative = \previous \cdot [ r ] \cdot \subsequent$} \label{alg:bayou:rbdeliver_tentative}
    \State{\Var $\newOrder = \committed \cdot \tentative$}
    \State{\Call{$\adjustExecution$}{$\newOrder$}}
\EndProcedure

\Upon{$\rbdeliver$}{$\langle\ISSUE, r$ : $\Request\rangle$} \label{alg:bayou:rbdeliver}
% \Upon{$\rbdeliver$}{$r$ : $\Request$} \label{alg:bayou:rbdeliver}
    \If{$r.\dot.\mathit{first} = i$}\LineComment{$r$ issued locally}
        \State{\Return}
    \EndIf
    \If{$\rr \not\in \committed$}
        \State{\Call{$\adjustTentativeOrder$}{$r$}} \label{alg:bayou:adjustTentativeOrder_late}
%         \State{\Var $\previous = [ x | x \in \tentative \wedge x < r ]$}
%         \State{\Var $\subsequent = [ x | x \in \tentative \wedge r < x ]$}    
%         \State{$\tentative = \previous \cdot [ r ] \cdot \subsequent$} \label{alg:bayou:rbdeliver_tentative}
%         \State{\Var $\newOrder = \committed \cdot \tentative$}
%         \State{\Call{$\adjustExecution$}{$\newOrder$}}
    \EndIf
\EndUpon

% \Upon{$\tobdeliver$}{$r$ : $\Request$} \label{alg:bayou:tobdeliver}
\Upon{$\tobdeliver$}{$\langle\COMMIT, r$ : $\Request\rangle$} \label{alg:bayou:rbdeliver}
%      \State{$\newTentative = [ x | x \in \tentative \wedge x \neq r ]$}
    \State{$\commit(r)$}
\EndUpon

\Procedure{$\commit$}{$r$ : $\Request$}
%      \If{$i = \primary$}
%         \State{\Return}
%      \EndIf
     \State{$\committed = \committed \cdot [ r ]$} \label{alg:bayou:tobdeliver_committed}
%      \State{$\tentative = \newTentative$}
    \State{$\tentative = [ x | x \in \tentative \wedge x \neq r ]$} \label{alg:bayou:tobdeliver_tentative}
% \columnbreak    
     \State{\Var $\newOrder = \committed \cdot \tentative$}
     \State{\Call{$\adjustExecution$}{$\newOrder$}}
     
     \If{$\requestsAwaitingResponse.\ccontains(r) \wedge r \in \executed$}
         \State{return $\requestsAwaitingResponse.\gget(r)$ to client} 
         \State{$\requestsAwaitingResponse.\rremove(r)$}
     \EndIf
\EndProcedure

% \Periodically{$\primarycommit()$}{} \label{alg:bayou:periodically}
%   \If{$i = \primary \wedge \tentative \neq []$}
%     \State{\Var $[\head] \cdot \tail = \tentative$}
%     \State{$\commit(\head)$}
%     \State{$\frbcast(\langle\COMMIT, \head\rangle)$}
%   \EndIf
% \EndPeriodically

\Procedure{$\adjustExecution$}{$\newOrder$ : list$\langle\Request\rangle$}
    \State{\Var $\inOrder =\ $longestCommonPrefix$(\executed, \newOrder)$}
    \State{\Var $\outOfOrder = [ x | x \in \executed \wedge x \not\in \inOrder ]$}
    
%     \If{$\inOrder \neq []$}
        \State{$\executed = \inOrder$}
        \State{$\toBeExecuted = [ x | x \in \newOrder \wedge x \not\in \executed ]$}
        \State{$\toBeRolledBack = \toBeRolledBack \cdot \reverse(\outOfOrder)$}
%     \EndIf
\EndProcedure

\Upon{$\toBeRolledBack \neq []$}{}
    \State{\Var $[ \head ] \cdot \tail = \toBeRolledBack$}
    \State{$\boxx.\rollback(\head)$} \label{alg:bayou:rollback}
    \State{$\toBeRolledBack = \tail$}
\EndUpon
    
\Upon{$\toBeRolledBack = [] \wedge \toBeExecuted \neq []$}{}
    \State{\Var $[ \head ] \cdot \tail = \toBeExecuted$}
    \State{\Var $\response = \boxx.\execute(\head)$} \label{alg:bayou:execute}
    
    \If{$\requestsAwaitingResponse.\ccontains(\head)$}
        \If{$\neg \head.\strongOp \vee \head \in \committed$}
            \State{return $\response$ to client}
             \State{$\requestsAwaitingResponse.\rremove(\head)$}
        \Else
           \State{$\requestsAwaitingResponse.\pput(\head, \response)$}
        \EndIf
    \EndIf
    
    \State{$\executed = \executed \cdot [ \head ]$}
    \State{$\toBeExecuted = \tail$}
\EndUpon

\end{algorithmic}
\end{multicols*}
\vspace{-0.4cm}
\end{algorithm*}

\endinput


\State{integer $\LC \gets 0$} \label{alg:htr:lc}
\State{set $\Log \gets \emptyset$} \label{alg:htr:log}

\Function{getObject}{txDescriptor $t$, objectId $\oid$}
  \If{$(\oid, \obj) \in t.\updates$} $\vvalue \gets \obj$ \label{alg:htr:retrieveUpdates}
  \State{\textbf{else} $\vvalue \gets$ retrieve object $\oid$} \label{alg:htr:retrieve}
  \EndIf
  \State{\Return $\vvalue$}
\EndFunction

\Function{certify}{integer $\start$, set $\readset$} \label{alg:htr:certify}
  \State{\LockStart $L \gets \{ {t \in \Log} : t.\eend > \start \}$ \LockEnd} 
\label{alg:htr:logFilter}
  %\For{$\forall_{t \in Log}\ t.end > start$}
  \ForAll{$t \in L$}
      \State{$\writeset \gets \{ \oid : \exists (\oid,\obj) \in t.\updates \}$}
      \If{$\readset \cap \writeset \neq \emptyset$} \Return $\failure$
      \EndIf
  \EndFor
  \State{\Return $\success$}
\EndFunction

\Procedure{updateOracleStatistics}{txDescriptor $t$} 
\label{alg:htr:updateOracle}
    \State{$\txoracle.\textproc{feed}(t.\stats)$}
\EndProcedure

\algrule

\item[\textbf{Thread $q$ on request} $r$ \textbf{from client} $c$ (executed on 
one replica)]
\State{enum $\outcome_q \gets \failure$}\hfill\textit{// type: enum \{ success, 
failure \}}
\State{response $\res_q \gets \nnull$}
\State{txDescriptor $\tdu \gets \nnull$}\hfill\textit{// type: (id, 
start, end, readset, updates, stats)} \label{alg:htr:txDesc}

\Upon{init}{}
  \State{\textbf{wait until} $\LC \ge r.\clock$} \label{alg:htr:clock}
  \State{\Call{Transaction()}{}}
  \State{\EndReq} 
\EndUpon

\Procedure{transaction}{}
% \While{$true$}{}
  \State{$\mode \gets \txoracle.\textproc{query}(r)$} \label{alg:htr:query}
  \If{$\mode = \mathit{DUmode}$} \label{alg:htr:dumode}
    \State{$\tdu \gets (\text{a new unique}\ \id, 0, 0, \emptyset, \emptyset, 
\emptyset)$}
    \State{\LockStart $\tdu.\start \gets \LC$ \LockEnd} \label{alg:htr:start}
    \State{$\res_q \gets$ execute $r.\prog$ with $r.\args$} \label{alg:htr:executeDU}
  \Else\hfill\textit{// mode = SMmode} \label{alg:htr:smmode}
    \State{\tobcast $r$}\hfill\textit{// blocking } \label{alg:htr:tobSM}
  \EndIf
  \If{$\outcome_q = \failure$} \Call{transaction()}{}
  \EndIf
%   \EndWhile
\EndProcedure

\Function{read}{objectId $\oid$} \label{alg:htr:DUFunctionsBegin}
    \State{$\tdu.\readset \gets \tdu.\readset \cup \{\oid\}$} 
\label{alg:htr:read}
    \State{\LockStart \textbf{if} \Call{certify}{$\tdu.\start, \{\oid\}$} $= 
\failure$ \textbf{then}} \Call{retry()}{}\label{alg:htr:check}
    \State{\AlgIndent \AlgIndentSmall \textbf{else} \Return \Call{getObject}{$\tdu$, $\oid$} 
\LockEnd} \label{alg:htr:getObjectCall}
\EndFunction

\Procedure{write}{objectId $\oid$, object $\obj$}
    \State{$\tdu.\updates \gets \{ (\oid',\obj') \in \tdu.\updates : \oid' \neq 
\oid \}$ \label{alg:htr:write}
    \item[] \AlgIndent\AlgIndent\AlgIndent $\cup\ \{(\oid,\ \obj)\}$} 
\EndProcedure

\Procedure{commit}{} \label{alg:htr:commit}
  \State \EndTxCode
  \If{$\tdu.\updates = \emptyset$} \label{alg:htr:noupdates}
    \State{$\outcome_q = \success$}
    \State \Return \label{alg:htr:noupdates2}
  \EndIf
  \If{\Call{certify}{$\tdu.\start, \tdu.\readset$} $= \failure$} \Return \label{alg:htr:localCert}
  \EndIf
  \State{\tobcast $\tdu$}\hfill\textit{// blocking} \label{alg:htr:tob}
  \State{\Call{updateOracleStatistics}{$\tdu$}} \label{alg:htr:updateOracleDU}
\EndProcedure

\Procedure{retry}{} \label{alg:htr:retry}
  \State{\EndTxCode}
\EndProcedure
% \algstore{myalg}
% \end{algorithmic}
% \end{algorithm}
% 
% \begin{algorithm}[h]
% \footnotesize
% \begin{algorithmic}[1]
% \algrestore{myalg}
% \item[]
\columnbreak
\Procedure{rollback}{} \label{alg:htr:rollback}
  \State{\EndTxCode}
  \State{$\outcome_q \gets \success$}
\EndProcedure \label{alg:htr:DUFunctionsEnd}

\algrule

\item[\textbf{The main thread of HTR} (executed on all replicas)]
\State{enum $\outcome \gets \nnull$}\hfill\textit{// type: enum \{ success, 
failure \}}
\State{response $\res \gets \nnull$}
\State{request $r \gets \nnull$}
\State{txDescriptor $\tsm \gets \nnull$} \label{alg:htr:txDesc2}

\Upon{\todeliver}{txDescriptor $\tdu$} \label{alg:htr:adeliverTx}
  \If{\Call{certify}{$\tdu.\start, \tdu.\readset$} $ = \success$} 
\label{alg:htr:globalCert}
     \State{\LockStart $\LC \gets \LC + 1$} \label{alg:htr:inc} \label{alg:htr:commitBegin} 
     \State{\AlgIndent $\tdu.\eend \gets \LC$ } \label{alg:htr:end} 
     \State{\AlgIndent $\Log \gets \Log \cup \{\tdu\}$} 
\label{alg:htr:logAppend}
     \State{\AlgIndent apply $\tdu.\updates$ \LockEnd} \label{alg:htr:apply}
\label{alg:htr:commitEnd}
  \If{transaction with $\tdu.\id$ executed locally by thread $q$} 
    \State{$\outcome_q \gets \success$}
  \EndIf
  \EndIf 
\EndUpon

\Upon{\todeliver}{request $r_q$} \label{alg:htr:adeliverTxSM}
  \State{$r \gets r_q$}
  \State{\Call{transaction()}{}}
  \State{\Call{updateOracleStatistics}{$\tsm$}} \label{alg:htr:updateOracleSM}
  \If{request with $r.\id$ handled locally by thread $q$}{}
    \State{$\osm \gets \outcome$}
    \State{$\res_q \gets \res$}
  \EndIf
\EndUpon

\Procedure{transaction}{}
  \State{$\tsm \gets (\text{a deterministic unique}\ \id \text{ based on 
$r.\id$}, 0, 0, \emptyset, \emptyset, \emptyset)$} \label{alg:htr:executionStartSM}
%   \State{\LockStart $\tsm.start \gets LC$ \LockEnd} \label{alg:htr:start}
  \State{$\tsm.start \gets LC$} \label{alg:htr:startSM}
  \State{$\res \gets \nnull$}
  \State{$\res \gets$ execute $r.\prog$ with $r.\args$} \label{alg:htr:executionEndSM}
\EndProcedure

\Function{read}{objectId $\oid$, object $\obj$} \label{alg:htr:SMFunctionsBegin}
%       \State{\LockStart $\vvalue \gets $ \Call{getObject}{$\tsm$, $\oid$} 
% \LockEnd } \label{alg:htr:getObjectCall}
%      \State{\Return $\vvalue$} 
     \State{\Return \Call{getObject}{$\tsm$, $\oid$}} \label{alg:htr:readSM}
\EndFunction

\Procedure{write}{objectId $\oid$, object $\obj$}
    \State{$\tsm.\updates \gets \{ (\oid',\obj') \in \tsm.\updates : \oid' \neq 
\oid \}$ \label{alg:htr:writeSM}
\item[] \AlgIndent\AlgIndent\AlgIndent $\cup\ \{(\oid,\ \obj)\}$} 
\EndProcedure

\Procedure{commit}{} \label{alg:htr:commitSM}
   \State \EndTxCode
   \If{$\tsm.\updates \neq \emptyset$} 
    \State{\LockStart $\LC \gets \LC + 1$} \label{alg:htr:incSM} \label{alg:htr:commitBeginSM}
    \State{\AlgIndent $\tsm.\eend \gets \LC$ } \label{alg:htr:endSM} 
        \State{\AlgIndent $\Log \gets \Log \cup \{\tsm\}$} 
    \label{alg:htr:logAppendSM}
        \State{\AlgIndent apply $\tsm.\updates$ \LockEnd} \label{alg:htr:applySM} \label{alg:htr:commitEndSM}
   \EndIf
   \State{$\outcome \gets \success$}
\EndProcedure

\Procedure{retry}{} \label{alg:htr:retrySM}
  \State \EndTxCode
  \State{$\outcome \gets \failure$}
\EndProcedure

\Procedure{rollback}{} \label{alg:htr:rollbackSM}
  \State \EndTxCode
  \State{$\outcome \gets \success$}
\EndProcedure \label{alg:htr:SMFunctionsEnd}
\vspace{-0.8cm}
\end{algorithmic}
\end{multicols*}
\vspace{-0.4cm}
\end{algorithm*}


==> algorithms/bayou_modified_alg.tex <==
\begin{algorithm}[t] 
\caption{Modification to Algorithm~\ref{alg:bayou} that prevents circular causality}
\label{alg:bayou_modified}  
% \algsetup{linenosize=\tiny}
  \footnotesize
% \vspace{-0.15cm}
% \begin{multicols*}{2}
\begin{algorithmic}[1]
\Upon{$\invoke$}{$\opn$ : $\ops(\FF)$, $\strongOp$ : boolean}
    \If{$\neg\strongOp \wedge \opn \in \readonlyops(\FF)$}
        \State{\Var $\response = \boxx.\execute(\opn)$}
        \State{return $\response$ to client}
    \Else
        \State{$\currentEventNumber = \currentEventNumber + 1$}
        \State{\Var $r = \Request(\currentTime, (i, \currentEventNumber), \strongOp, \opn)$}
        \If{$\neg\strongOp$}
            \State{\Var $\response = \boxx.\execute(r)$}
            \State{return $\response$ to client}
            \State{$\boxx.\rollback(r)$}
            \State{$\rbcast(r)$}
            \State{$\tobcast(r)$}
            \State{\Call{$\adjustTentativeOrder$}{$r$}}
        \Else
            \State{$\requestsAwaitingResponse.\pput(r, \bot)$}
            \State{$\tobcast(r)$}
        \EndIf
\EndUpon\end{algorithmic}
% \end{multicols*}
% \vspace{-0.4cm}
\end{algorithm}

\endinput





\begin{algorithm}[t] 
\caption{Modification to Algorithm~\ref{alg:bayou} that prevents circular causality}
\label{alg:bayou_modified}  
% \algsetup{linenosize=\tiny}
  \footnotesize
% \vspace{-0.15cm}
% \begin{multicols*}{2}
\begin{algorithmic}[1]
\Upon{$\invoke$}{$\opn$ : $\ops(\FF)$, $\strongOp$ : boolean}
    \State{$\currentEventNumber = \currentEventNumber + 1$}
    \State{\Var $r = \Request(\currentTime, (i, \currentEventNumber), \strongOp, \opn)$}
    \If{$\neg\strongOp$}
        \State{\Var $\response = \boxx.\execute(r)$}
        \State{return $\response$ to client}
        \State{$\boxx.\rollback(r)$}
        \If{$\opn \not\in \readonlyops(\FF)$}
            \State{$\rbcast(r)$}
            \State{$\tobcast(r)$}
            \State{\Call{$\adjustTentativeOrder$}{$r$}}
        \EndIf
    \Else
        \State{$\requestsAwaitingResponse.\pput(r, \bot)$}
        \State{$\tobcast(r)$}
    \EndIf
\EndUpon\end{algorithmic}
% \end{multicols*}
% \vspace{-0.4cm}
\end{algorithm}



==> algorithms/seq_redblue.tex <==
\begin{algorithm}[t] 
\caption{RedBlue-consistent implementation of a replicated sequence for replica $R_i$}
\label{alg:seq_redblue}  
% \algsetup{linenosize=\tiny}
  \footnotesize
% \vspace{-0.15cm}
% \begin{multicols*}{2}
\begin{algorithmic}[1]
\State{\Struct $\Request$($s$ : string, $\lc$ : int)}
\Operator{$<$}{$\rr : \Request$, $\rr' : \Request$}
    \State{\Return $(\rr.\lc, \rr.s) < (\rr'.\lc, \rr.s)$}
\EndOperator         
         
\State{\Var $\lc$ : int} 
\State{\Var $\delReqs$ : set$\langle\Request\rangle$}
\Function{$\blueapp$}{$s$ : string}
     \State{\Var $r = \Request(s, \lc)$} \LineComment{$\blueapp$ generator operation}
     \State{issue blue shadow operation $\mathit{appendShadow}(r)$}
     \State{\Return $\ok$}
\EndFunction
\Function{$\redapp$}{$s$ : string}
     \State{\Var $r = \Request(s, \lc)$} \LineComment{$\redapp$ generator operation}
     \State{issue red shadow operation $\mathit{appendShadow}(r)$}
     \State{\Return $\ok$}
\EndFunction
% \Function{$\mathit{appendGenerator}$}{$s$ : string, $\type$ : $\{$RED, BLUE$\}$} 
%     \State{\Var $r = \Request(s, \lc)$}
%     \If{$\type =\ $RED}
%         \State{issue red shadow operation $\mathit{appendShadow}(r)$}
%     \Else
%         \State{issue blue shadow operation $\mathit{appendShadow}(r)$}
%     \EndIf
% \EndFunction
\Function{$\mathit{appendShadow}$}{$r$ : $\Request$} % \LineComment{$\blueapp$ and $\redapp$ shadow operation}
    \State{$\lc = \max(\lc, r.\lc) + 1$}
    \State{$\delReqs = \delReqs \cup \{ r \}$}
\EndFunction
\Function{$\bluerd()$}{}
    \State{\Var $\seq = \epsilon$}
    \For{$r$ \textbf{in} $\sort(\delReqs)$} \LineComment{sorted by $\lc$ and $s$}
        \State{$\seq = \seq \cdot r.s$}
    \EndFor
    \State{\Return $\seq$}
\EndFunction
\end{algorithmic}
\end{algorithm}

\endinput

\begin{algorithm}[t] 
\caption{RedBlue-consistent implementation of a replicated sequence for replica $R_i$}
\label{alg:seq_redblue}  
% \algsetup{linenosize=\tiny}
  \footnotesize
% \vspace{-0.15cm}
% \begin{multicols*}{2}
\begin{algorithmic}[1]
% \State{\Struct $\Message$($\type$ : ${\{}$ ADD, SUBTRACT ${\}}$, $\value$ : int)}
\State{\Struct $\Request$($\type$ : ${\{}$RED, BLUE${\}}$, $s$ : string, $\timestamp$ : int, \par
         \hskip 3.2em $\idd$ : pair$\langle$int, int$\rangle$)}
\Operator{$<$}{$\rr : \Request$, $\rr' : \Request$}
    \State{\Return $(\rr.\timestamp, \rr.\dot) < (\rr'.\timestamp, \rr'.\dot)$}
\EndOperator         
         
% \State{\Var $\seq$ : string} \label{alg:actpc:vars}
\State{\Var $\delReqs$ : set$\langle\Request\rangle$}
% \State{\Var $\requestsAwaitingResponse$ : set$\langle$pair$\langle$int, int$\rangle\rangle$}

\Function{$\blueapp$}{$s$ : string} \LineComment{blue operation} \label{alg:actpc:add}
    \State{$\currentEventNumber = \currentEventNumber + 1$}
    \State{$r = \Request($BLUE, $s, \currentTime, (i, \currentEventNumber))$}
    \State{$\rbcast(r)$} \label{alg:actpc:addrb}
    \State{\Return $\ok$}
\EndFunction
\Function{$\redapp$}{$s$ : string} \LineComment{red operation} \label{alg:actpc:add}
    \State{$\currentEventNumber = \currentEventNumber + 1$}
    \State{$r = \Request($RED, $s, \currentTime, (i, \currentEventNumber))$}
    \State{$\tobcast(r)$} \label{alg:actpc:addrb}
    \State{\Return $\ok$}
\EndFunction
\Upon{$\rbdeliver$}{$r$ : $\Request($BLUE, $s, \timestamp, \idd)$} 
    \State{$\delReqs = \delReqs \cup \{ r \}$}
\EndUpon
\Upon{$\tobdeliver$}{$r$ : $\Request($RED, $s, \timestamp, \idd)$} 
    \State{$\delReqs = \delReqs \cup \{ r \}$}
\EndUpon
\Function{$\rd()$}{} \LineComment{blue operation} \label{alg:actpc:subtract}
    \State{\Var $\seq = \bot$}
    \For{$r : \delReqs$} 
        \State{$\seq = \seq \cdot r.s$}
    \EndFor
    \State{\Return $\seq$}
\EndFunction
\end{algorithmic}
\end{algorithm}

\endinput



\Function{$\rollback$}{$r$ : $\Request$}
    \State{\Var $\undoMap = \undoLog[r]$}
    \For{$(k,v) \in \undoMap$}
        \State{$\db[k] = v$}
        \State{$\undoLog = \undoLog \setminus (r, \undoMap)$}
    \EndFor
\EndFunction
\end{algorithmic}
% \end{multicols*}
% \vspace{-0.4cm}
\end{algorithm}

\endinput




==> histories/bayou_history.tex <==
\begin{tikzpicture}[font=\sf\footnotesize] 

\tikzstyle{time line} = [->, thick];
\tikzstyle{bcast line} = [->, dashed, thick];
\tikzstyle{tobcast line} = [->];
\tikzstyle{dot} = [circle, fill, inner sep=1pt];

\newcommand{\dist}{1.15}
\newcommand{\procdist}{2.3}
\newcommand{\tlength}{0.4}
\newcommand{\mypattern}{north west lines}

\node (r1) at (0, 1 * \procdist) [left] {$R_1$};
\node (r2) at (0, 0.5 * \procdist) [left] {$R_2$};
\node (r3) at (0, 0.0 * \procdist) [left] {$\mathit{(primary)}\ R_3$};

\draw [time line] (r1) -- (7.15 * \dist, 1 * \procdist);
\draw [time line] (r2) -- (7.15 * \dist, 0.5 * \procdist);
\draw [time line] (r3) -- (7.15 * \dist, 0.0 * \procdist);

% % % % 
% R1

\abdotname{it1}{1.0 * \dist, 1.0 * \procdist}{$\invoke(T_1)$};

\emptydot{r1rect2}{1.3 * \dist, 1.0 * \procdist};

\emptydot{r1t2}{1.6 * \dist, 1.0 * \procdist};
\emptydot{r1t2e}{$(r1t2) + (\tlength, 0)$};
\mysegfill{r1t2}{r1t2e};

\emptydot{r1t1}{2.1 * \dist, 1.0 * \procdist};
\emptydot{r1t1e}{$(r1t1) + (\tlength, 0)$};
\mysegdraw{r1t1}{r1t1e};

\beldotname{iq}{2.8 * \dist, 1.0 * \procdist}{$\invoke(Q_1)$};

\emptydot{r1q}{2.9 * \dist, 1.0 * \procdist};
\emptydot{r1qe}{$(r1q) + (\tlength, 0)$};
\mysegfillcustom{r1q}{r1qe}{\mypattern};

\abdotname{responseQ}{3.4 * \dist, 1.0 * \procdist}{$\responserm(Q_1{,} 1)$};

\emptydot{r1recct1}{3.8 * \dist, 1.0 * \procdist};
\emptydot{r1recct2}{5.0 * \dist, 1.0 * \procdist};


\emptydot{r1t1r}{3.95 * \dist, 1.0 * \procdist};
\emptydot{r1t1re}{$(r1t1r) + (\tlength, 0)$};
\mysegdraw{r1t1r}{r1t1re};

\emptydot{r1t2r}{4.45 * \dist, 1.0 * \procdist};
\emptydot{r1t2re}{$(r1t2r) + (\tlength, 0)$};
\mysegfill{r1t2r}{r1t2re};


% % % % 
% R2

\beldotname{it2}{0.5 * \dist, 0.5 * \procdist}{$\invoke(T_2)$};

\emptydot{r2rect1}{1.25 * \dist, 0.5 * \procdist};

\emptydot{r2recct1}{2.8 * \dist, 0.5 * \procdist};
\emptydot{r2recct2}{4.0 * \dist, 0.5 * \procdist};

\emptydot{r2t1}{4.5 * \dist, 0.5 * \procdist};
\emptydot{r2t1e}{$(r2t1) + (\tlength, 0)$};
\mysegdraw{r2t1}{r2t1e};

\emptydot{r2t2}{5.0 * \dist, 0.5 * \procdist};
\emptydot{r2t2e}{$(r2t2) + (\tlength, 0)$};
\mysegfill{r2t2}{r2t2e};

\beldotname{invokeQ}{5.7 * \dist, 0.5 * \procdist}{$\invoke(Q_2)$};

\emptydot{r2q}{5.8 * \dist, 0.5 * \procdist};
\emptydot{r2qe}{$(r2q) + (\tlength, 0)$};
\mysegfillcustom{r2q}{r2qe}{\mypattern};

\abdotname{responseQ}{6.3 * \dist, 0.5 * \procdist}{$\responserm(Q_2{,} 2)$};

% % % % 
% R3

\emptydot{r3t1}{2.0 * \dist, 0.0 * \procdist};
\emptydot{r3t1e}{$(r3t1) + (\tlength, 0)$};
\mysegdraw{r3t1}{r3t1e};

\beldotname{ct1}{2.5 * \dist, 0.0 * \procdist}{$\commit(T_1)$};

\emptydot{r3t2}{3.2 * \dist, 0.0 * \procdist};
\emptydot{r3t2e}{$(r3t2) + (\tlength, 0)$};
\mysegfill{r3t2}{r3t2e};

\beldotname{ct2}{3.7 * \dist, 0.0 * \procdist}{$\commit(T_2)$};

% % % 

\draw [tobcast line] (it1.center) -- (r2rect1.center);
\draw [tobcast line] (it1.center) -- (r3t1.center);

\draw [tobcast line] (it2.center) -- (r1rect2.center);
\draw [tobcast line] (it2.center) -- (r3t2.center);

\draw [tobcast line] (ct1.center) -- (r1recct1.center);
\draw [tobcast line] (ct1.center) -- (r2recct1.center);

\draw [tobcast line] (ct2.center) -- (r1recct2.center);
\draw [tobcast line] (ct2.center) -- (r2recct2.center);

% % % 

\begin{scope}[shift={(-0.1, 0.3)}]
\emptydot{a1}{0, -1};
\emptydot{a1e}{0.4, -1};
\mysegdraw{a1}{a1e};
\node (t1) at (1.4, -1.0) {$\mathit{executions\ of\ T_1}$};

\emptydot{a1}{2.9, -1};
\emptydot{a1e}{3.3, -1};
\mysegfill{a1}{a1e};
\node (t1) at (4.3, -1) {$\mathit{executions\ of\ T_2}$};

\emptydot{a1}{5.7, -1};
\emptydot{a1e}{6.1, -1};
\mysegfillcustom{a1}{a1e}{\mypattern};
\node (t1) at (7.3, -1) {$\mathit{executions\ of\ Q_1/Q_2}$};
\end{scope}


\end{tikzpicture}

\endinput

\begin{scope}[shift={(-0.5,0)}]
\emptydot{append}{1.0 * \dist, 1.0 * \procdist};    
\emptydot{r1p}{2.6 * \dist, 1.0 * \procdist};
\emptydot{r1}{3.0 * \dist, 1.0 * \procdist};
\emptydot{r2}{4.0 * \dist, 1.0 * \procdist};
\emptydot{r2e}{4.2 * \dist, 1.0 * \procdist};
% \mysegdraw{$(r2)$}{$(r2e)$};
\emptydot{q1}{2.5 * \dist, 0.5 * \procdist};
\emptydot{q1e}{2.9 * \dist, 0.5 * \procdist};
\mysegdraw{$(q1)$}{$(q1e)$};
\emptydot{q2}{3.5 * \dist, 0.5 * \procdist};
\emptydot{q2e}{3.7 * \dist, 0.5 * \procdist};
% \mysegdraw{$(q2)$}{$(q2e)$};

% \draw [bcast line] (append) to [bend left] (r1);
\mysegfill{$(r1p)$}{$(r1)$};
\draw [tobcast line] (append.center) to [bend left] (r2.center);
\draw [bcast line] (append.center) to (q1.center);
\draw [tobcast line] (append.center) to (q2.center);

\absegarbdashed{1.0 * \dist, 1.3 * \procdist}{2 * \dist,0}{$\append(a) \rightarrow a\ (\rightarrow a)$}{2.6 * \dist, 1.3 * \procdist};
\absegarb{3.0 * \dist, 1.3 * \procdist}{1 * \dist,0}{}{0,0};
\end{scope}
 
\begin{scope}[shift={(4.5,0)}]
    


\emptydot{append}{1.0 * \dist, 1.0 * \procdist};
\emptydot{replace}{0.5 * \dist, 0.5 * \procdist};

\emptydot{r1}{2.0 * \dist, 1.0 * \procdist};
\emptydot{r1e}{2.4 * \dist, 1.0 * \procdist};
\mysegdraw{$(r1)$}{$(r1e)$};
\emptydot{r2p}{2.6 * \dist, 1.0 * \procdist};
\emptydot{r2}{3.0 * \dist, 1.0 * \procdist};
\mysegfill{$(r2p)$}{$(r2)$};
\emptydot{r3}{3.6 * \dist, 1.0 * \procdist};
\emptydot{r3e}{4.0 * \dist, 1.0 * \procdist};
\mysegdraw{$(r3)$}{$(r3e)$};
\emptydot{r4}{5.0 * \dist, 1.0 * \procdist};
\emptydot{r4e}{5.4 * \dist, 1.0 * \procdist};
\mysegdraw{$(r4)$}{$(r4e)$};

\emptydot{q1}{1.5 * \dist, 0.5 * \procdist};
\emptydot{q1e}{1.9 * \dist, 0.5 * \procdist};
\mysegdraw{$(q1)$}{$(q1e)$};
% \emptydot{q2}{2.5 * \dist, 0.5 * \procdist}{};
\emptydot{q3}{3.5 * \dist, 0.5 * \procdist};
\emptydot{q3e}{3.7 * \dist, 0.5 * \procdist};
% \mysegdraw{$(q3)$}{$(q3e)$};
\emptydot{q4}{4.5 * \dist, 0.5 * \procdist};
\emptydot{q4p}{4.3 * \dist, 0.5 * \procdist};
\emptydot{q4e}{4.7 * \dist, 0.5 * \procdist};
\mysegfill{$(q4p)$}{$(q4e)$};

% \draw [bcast line] (append) to [bend left] (r2);
% \mysegfill{$(append)$}{$(r2)$};
\draw [tobcast line] (append.center) to [bend left] (r3.center);
\draw [bcast line] (replace.center) to (r1.center);
\draw [tobcast line] (replace.center) to (r4.center);

\draw [bcast line] (append.center) to (q1.center);
\draw [tobcast line] (append.center) to (q3.center);
% \draw [bcast line] (replace) to [bend right] (q2);
% \mysegfill{$(replace)$}{$(q4)$};
\draw [tobcast line] (replace.center) to [bend right] (q4.south);

\absegarbdashed{1.0 * \dist, 1.3 * \procdist}{2 * \dist,0}{$\append(x) \rightarrow aax\ (\rightarrow ax)$}{2.6 * \dist, 1.3 * \procdist};
\absegarb{3.0 * \dist, 1.3 * \procdist}{1 * \dist,0}{}{0,0};

\belsegarb{0.5 * \dist, 0.15 * \procdist}{4 * \dist,0}{$\duplicate() \rightarrow axax$}{2.5 * \dist, 0.15 * \procdist};

\end{scope}

\begin{scope}[shift={(12,2.5)}]
\draw [bcast line] (0, 0) -- (1, 0) {};
\node (t1) at (3.4, 0) {$\mathit{message\ broadcast\ through\ RB}$};

\draw [tobcast line] (0, -0.5) -- (1, -0.5) {};
\node (t1) at (3.5, -0.5) {$\mathit{message\ broadcast\ through\ TOB}$};

\emptydot{a1}{0, -1};
\emptydot{a1e}{1, -1};
\mysegfill{$(a1)$}{$(a1e)$};
\node (t1) at (3.97, -1.0) {$\mathit{executions\ that\ return\ values\ to\ clients}$};

\emptydot{a1}{0, -1.5};
\emptydot{a1e}{1, -1.5};
\mysegdraw{$(a1)$}{$(a1e)$};
\node (t1) at (2.34, -1.5) {$\mathit{other\ executions}$};
\end{scope}

% \node (high) at (0.2 * \dist, 1.2 * \procdist) {};
% \node (low) at (0.2 * \dist, 0.25 * \procdist) {};
% 
% \node (high label) at (0.2 * \dist, 1.3 * \procdist) {$\mathit{stable\ state} : a$};
% 
% \draw [dashed] (high) -- (low);

% \beldotname{order}{5.7 * \dist, 0.5 * \procdist}{};
% 
% \belleftsegarbdashed{5.7 * \dist, 0.15 * \procdist}{0.7 * \dist,0}{$\mathit{order}(pizza{,} 210) \rightarrow ...$}{6.2 * \dist, 0.15 * \procdist};


% \abdotname{r1}{2.0 * \dist, 1.0 * \procdist}{};
% \abdotname{r2}{2.0 * \dist, 1.0 * \procdist}{};
% \abdotname{r3}{2.0 * \dist, 1.0 * \procdist}{};
% \abdotname{r4}{2.0 * \dist, 1.0 * \procdist}{};


% \abdot{3.0 * \dist, 1.0 * \procdist}{};
% \abdot{4.0 * \dist, 1.0 * \procdist}{};
% \abdot{5.0 * \dist, 1.0 * \procdist}{};

%  \abdot{3.5 * \dist, 1.0 * \procdist}{$\rd() \rightarrow 3$};
% \abdot{5.5 * \dist, 1.0 * \procdist}{$\rd() \rightarrow 3$};
% 

% 
% \node (dots1) at (6.45 * \dist, 1.0 * \procdist + 0.3) {$...$};
% % \node (dots2) at (7.5 * \dist, 0.1) {$...$};
% 
% \draw [time line] (0.5 * \dist, 0.5 * \procdist) -- (1 * \dist, 1.0 * \procdist);


